Energy-frugal and Interpretable AI Hardware Design using Learning Automata

Energy efficiency is a crucial requirement for enabling powerful artificial intelligence applications at the microedge. Hardware acceleration with frugal architectural allocation is an effective method for reducing energy. Many emerging applications also require the systems design to incorporate interpretable decision models to establish responsibility and transparency. The design needs to provision for additional resources to provide reachable states in real-world data scenarios, defining conflicting design tradeoffs between energy efficiency. is challenging. Recently a new machine learning algorithm, called the Tsetlin machine, has been proposed. The algorithm is fundamentally based on the principles of finite-state automata and benefits from natural logic underpinning rather than arithmetic. In this paper, we investigate methods of energy-frugal artificial intelligence hardware design by suitably tuning the hyperparameters, while maintaining high learning efficacy. To demonstrate interpretability, we use reachability and game-theoretic analysis in two simulation environments: a SystemC model to study the bounded state transitions in the presence of hardware faults and Nash equilibrium between states to analyze the learning convergence. Our analyses provides the first insights into conflicting design tradeoffs involved in energy-efficient and interpretable decision models for this new artificial intelligence hardware architecture. We show that frugal resource allocation coupled with systematic prodigality between randomized reinforcements can provide decisive energy reduction while also achieving robust and interpretable learning.

==> future.tex <==
\section{Future Work}

Pervasive:
Low-power

Scale-up:
Memory
Architecture



==> texmf/tex/latex/common/pgflibraryshapes.gates.logic.comparator.code.tex <==
\usepgflibrary{shapes.gates.logic}
\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
	comparator symbol/.initial=,
}

% Shape comparator
%
\pgfdeclareshape{comparator}{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@comparator\endcsname{%
    \pgf@lib@sh@logicgate@parseinputs{2}%
    \pgfmathloop%
    \ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
    \else%
            \pgfutil@ifundefined{pgf@anchor@comparator@input \pgfmathcounter}{%
                    \expandafter\xdef\csname pgf@anchor@comparator@input \pgfmathcounter\endcsname{%
                            \noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
                    }%
            }{}%
    \repeatpgfmathloop%
    \ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
      \pgferror{A comparator must have two inputs}%
    \fi%
  }%
  \savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
  \saveddimen\invertedradius{%
          \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
  }%
  \saveddimen\outerinvertedradius{%
          \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
          \advance\pgf@x.5\pgflinewidth%
  }
  \saveddimen\halflinewidth{%
    \pgf@x.5\pgflinewidth%
  }%
  \savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}%
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }%
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+0.5ex}%
  }%
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}%
  \anchor{mid east}{%
    \midpoint%
    \pgfutil@tempdima\pgf@y%
    \csname pgf@anchor@comparator@east\endcsname%
    \pgf@y\pgfutil@tempdima%
  }%
  \anchor{mid west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \midpoint%
    \advance\pgf@x\pgf@xc%
  }%
  \anchor{base}{\basepoint}%
  \anchor{base east}{%
    \basepoint%
    \pgfutil@tempdima\pgf@y%
    \csname pgf@anchor@comparator@east\endcsname%
    \pgf@y\pgfutil@tempdima%
  }%
  \anchor{base west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \basepoint%
    \advance\pgf@x\pgf@xc%
  }%
  \inheritanchor[from=and gate US]{base}%
  \anchor{output}{%
    \dimensions%
    \pgf@xc\halfside%
    \centerpoint%
    \advance\pgf@x-.166666\pgf@xc%
    \pgf@xc2.0\pgf@xc%
    \advance\pgf@x.866025\pgf@xc%
    \advance\pgf@x\outerxsep%
  }%
  \anchor{east}{%
    \dimensions%
    \tipanchor%
    \pgf@xa\pgf@x%
    \centerpoint%
    \advance\pgf@x\pgf@xa%
  }%
  \anchor{north}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@north west\endcsname%
      \pgf@ya\pgf@y%
      \centerpoint%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y1pt}%
      {\csname pgf@anchor@comparator@north west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@south west\endcsname%
      \pgf@ya\pgf@y%
      \centerpoint%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y-1pt}%
      {\csname pgf@anchor@comparator@south west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south east}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@south west\endcsname%
      \pgf@ya\pgf@y%
      \pgf@process{%
        \dimensions%
        \tipanchor%
        \pgf@xa\pgf@x%
        \centerpoint%
        \advance\pgf@x\pgf@xa%
      }%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y-1pt}%
      {\csname pgf@anchor@comparator@south west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{north east}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@north west\endcsname%
      \pgf@ya\pgf@y%
      \pgf@process{%
        \dimensions%
        \tipanchor%
        \pgf@xa\pgf@x%
        \centerpoint%
        \advance\pgf@x\pgf@xa%
      }%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y1pt}%
      {\csname pgf@anchor@comparator@north west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south west}{%
    \dimensions%
    \pgf@xa\halfside%
    \centerpoint%
    \advance\pgf@x-.833333\pgf@xa
    \advance\pgf@x-\outerxsep%
    \advance\pgf@y-1.166666\pgf@xa%
    \pgf@ya\outerysep%
    \advance\pgf@y-1.565\pgf@ya% Selected by trial and error.
  }%
  \anchor{north west}{%
    \dimensions%
    \pgf@xa\halfside%
    \centerpoint%
    \advance\pgf@x-.833333\pgf@xa
    \advance\pgf@x-\outerxsep%
    \advance\pgf@y1.166666\pgf@xa%
    \pgf@ya\outerysep%
    \advance\pgf@y1.565\pgf@ya% Selected by trial and error.
  }%
  \anchor{west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \centerpoint%
    \advance\pgf@x\pgf@xc%
  }%
  \backgroundpath{%
    \dimensions%
    \pgf@xc\halfwidth%
    \pgf@yc\halfheight%
    \advance\pgf@xc-\outerxsep%
    \advance\pgf@yc-\outerysep%
    {%
	\pgftransformshift{\centerpoint}%
	\pgfpathmoveto{\tipanchor}%
	\pgfpathlineto{\pgfpoint{-\pgf@xc}{-\pgf@yc}}
	\pgfpathlineto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
	\pgfpathlineto{\tipanchor}%

	%
	% Draw inputs.
	%
	\pgf@xc-\halfwidth%
	\advance\pgf@xc-\invertedradius%
	\pgf@yc\halfheight%
	\pgfutil@tempdima2.0\pgf@yc%
	\c@pgf@counta\numinputs%
	\advance\c@pgf@counta1\relax%
	\divide\pgfutil@tempdima\c@pgf@counta%
	\pgfmathloop%
	\ifnum\pgfmathcounter>\numinputs%
	\else%
		\advance\pgf@yc-\pgfutil@tempdima%
		\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
			{%
				\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
			}%
		\fi%
	\repeatpgfmathloop%
    }%
  }%
  \anchorborder{%
    \pgf@lib@gates@not@buffer@border{comparator}
  }%

}%


\endinput


==> texmf/tex/latex/common/pgflibraryshapes.gates.logic.mux.code.tex <==
% Copyright 2008 by Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{shapes.gates.logic}
\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
	mux symbol/.initial=,
}

% Shape mux
%
\pgfdeclareshape{mux}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@mux\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@mux@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@mux@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A mux must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{mux}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}
	\anchor{mid west}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{mid east}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x\halfwidth}%
	\anchor{base}{\basepoint}
	\anchor{base west}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{base east}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x\halfwidth}%
	\anchor{north}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%
	\anchor{south}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%
	\anchor{east}{\dimensions\centerpoint\advance\pgf@x\halfwidth}%
	\anchor{west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth}%
	\anchor{north east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by -\pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
	\anchor{north west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y\halfheight}%
	\anchor{south east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by \pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
	\anchor{south west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y-\halfheight}%

	\anchor{select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%

	\anchor{other select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%

	\anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 

	\anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 

  \backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\pgfmathaddtolength\pgf@xc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@yc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		{%
			\pgftransformshift{\centerpoint}%

      \pgfmathadd{\pgf@yc}{-1.155\pgf@xc}
      \let\pgf@yd\pgfmathresult

      \pgfpathmoveto{\pgfpoint{-\pgf@xc}{-\pgf@yc}}
			\pgfpathlineto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
  		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yd}}
  		\pgfpathlineto{\pgfpoint{\pgf@xc}{-\pgf@yd}}
      \pgfpathclose

			%
			% Draw inputs.
			%
			\pgf@xc-\halfwidth%
			\advance\pgf@xc-\invertedradius%
			\pgf@yc\halfheight%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
					}%
				\fi%
			\repeatpgfmathloop%
		}%
  }

	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{mux}}

	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\dimensions%
		\pgfpointadd{\centerpoint}{\pgfpointborderrectangle{\externalpoint}{\pgfqpoint{\halfwidth}{\halfheight}}}%
	}%	

}


\endinput


==> texmf/tex/latex/common/tikzlibrarycircuits.logic.comparator.code.tex <==
\usetikzlibrary{circuits.logic}
\usepgflibrary{shapes.gates.logic.comparator}

\tikzset{
  circuit declare symbol = comparator,
}

\tikzset{
 set comparator graphic={
   circuit symbol open,
   circuit symbol size=width 0 height 4,
   shape=comparator,
   inner sep=.5ex
 }
}

\endinput


==> texmf/tex/latex/common/tikzlibrarycircuits.logic.mux.code.tex <==
% Copyright 2008 by Till Tantau and Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{circuits.logic}
\usepgflibrary{shapes.gates.logic.mux}

\tikzset{
  circuit declare symbol = mux,
}

\tikzset{
 set mux graphic={
   circuit symbol open,
   circuit symbol size=width 2.5 height 6,
   shape=mux,
   inner sep=.5ex
 }
}

\endinput

